Combining Diverse Feature Priors

To improve model generalization, model designers often restrict the features that their models use, either implicitly or explicitly. In this work, we explore the design space of leveraging such feature priors by viewing them as distinct perspectives on the data. Specifically, we find that models trained with diverse sets of feature priors have less overlapping failure modes, and can thus be combined more effectively. Moreover, we demonstrate that jointly training such models on additional (unlabeled) data allows them to correct each other's mistakes, which, in turn, leads to better generalization and resilience to spurious correlations. Code available at https://github.com/MadryLab/copriors

==> figures/basic_table_STLSub10_pureB.tex <==
\begin{tabular}{llccc}
\toprule
                                  Method &  Prior(s) &               Labeled only &                 \begin{tabular}{c}+Unlabeled \\Self/Co-Training\end{tabular}&                          \begin{tabular}{c} + Standard model \\with Pseudo-labels \end{tabular} \\
\midrule
      \multirow{4}{*}{Self-training} &   Standard &           53.73 $\pm$ 0.93 &           60.79 $\pm$ 0.91 &                            60.53 $\pm$ 0.90 \\
                                     &      Canny &  \textbf{56.24 $\pm$ 0.91} &           59.18 $\pm$ 0.90 &                            62.19 $\pm$ 0.91 \\
                                     &     BagNet &           52.04 $\pm$ 0.91 &           60.50 $\pm$ 0.92 &                            61.69 $\pm$ 0.91 \\
 \midrule \multirow{4}{*}{Standard co-training} &   Standard &           53.73 $\pm$ 0.92 &           60.46 $\pm$ 0.88 &           \multirow{2}{*}{61.23 $\pm$ 0.90} \\
                                     &  +Standard &  \textbf{55.38 $\pm$ 0.93} &           60.56 $\pm$ 0.90 &                                             \\
                         \cline{2-5} &      Canny &  \textbf{56.24 $\pm$ 0.92} &           62.86 $\pm$ 0.91 &  \multirow{2}{*}{\textbf{67.33 $\pm$ 0.90}} \\
                                     &    +BagNet &           52.04 $\pm$ 0.93 &  \textbf{66.74 $\pm$ 0.91} &                                             \\
                                     \midrule

 \multirow{4}{*}{Disjoint co-training} &   Standard &           53.73 $\pm$ 0.91 &           60.51 $\pm$ 0.90 &           \multirow{2}{*}{61.64 $\pm$ 0.90} \\
                                     &  +Standard &  \textbf{55.38 $\pm$ 0.92} &           60.55 $\pm$ 0.93 &                                             \\
                         \cline{2-5} &      Canny &  \textbf{56.24 $\pm$ 0.91} &           63.03 $\pm$ 0.89 &  \multirow{2}{*}{\textbf{67.11 $\pm$ 0.86}} \\
                                     &    +BagNet &           52.04 $\pm$ 0.91 &  \textbf{66.03 $\pm$ 0.86} &                                             \\
\bottomrule
\end{tabular}


==> figures/basic_table_STLSub10_pureT.tex <==
\begin{tabular}{llccc}
\toprule
                                  Method &  Prior(s) &               Labeled only &                 \begin{tabular}{c}+Unlabeled \\Self/Co-Training\end{tabular}&                          \begin{tabular}{c} + Standard model \\with Pseudo-labels \end{tabular} \\
\midrule
      \multirow{4}{*}{Self-training} &   Standard &           53.73 $\pm$ 0.92 &           60.79 $\pm$ 0.91 &                            60.53 $\pm$ 0.90 \\
                                     &      Canny &  \textbf{56.24 $\pm$ 0.90} &           59.18 $\pm$ 0.91 &                            62.19 $\pm$ 0.91 \\
                                     &      Sobel &  \textbf{55.56 $\pm$ 0.91} &           59.73 $\pm$ 0.91 &                            60.93 $\pm$ 0.90 \\
                                     &     BagNet &           52.04 $\pm$ 0.90 &           60.50 $\pm$ 0.92 &                            61.69 $\pm$ 0.90 \\
 \midrule \multirow{6}{*}{Co-training} &   Standard &           53.73 $\pm$ 0.91 &           60.51 $\pm$ 0.90 &           \multirow{2}{*}{61.64 $\pm$ 0.90} \\
                                     &  +Standard &  \textbf{55.38 $\pm$ 0.92} &           60.55 $\pm$ 0.93 &                                             \\
                         \cline{2-5} &      Canny &  \textbf{56.24 $\pm$ 0.91} &           63.03 $\pm$ 0.89 &  \multirow{2}{*}{\textbf{67.11 $\pm$ 0.86}} \\
                                     &    +BagNet &           52.04 $\pm$ 0.91 &  \textbf{66.03 $\pm$ 0.86} &                                             \\
                         \cline{2-5} &      Sobel &  \textbf{55.56 $\pm$ 0.89} &           62.60 $\pm$ 0.93 &           \multirow{2}{*}{65.80 $\pm$ 0.89} \\
                                     &    +BagNet &           52.04 $\pm$ 0.90 &           64.94 $\pm$ 0.88 &                                             \\
\bottomrule
\end{tabular}


==> figures/basic_table_cifarsmallsub_pureB.tex <==
\begin{tabular}{llccc}
\toprule
                                  Method &  Prior(s) &               Labeled only &                 \begin{tabular}{c}+Unlabeled \\Self/Co-Training\end{tabular}&                          \begin{tabular}{c} + Standard model \\with Pseudo-labels \end{tabular} \\
\midrule
      \multirow{4}{*}{Self-training} &   Standard &  \textbf{52.50 $\pm$ 0.81} &           64.61 $\pm$ 0.79 &                            64.01 $\pm$ 0.80 \\
                                     &      Sobel &  \textbf{51.93 $\pm$ 0.82} &           63.63 $\pm$ 0.80 &                            64.87 $\pm$ 0.79 \\
                                     &     BagNet &           44.48 $\pm$ 0.83 &           63.77 $\pm$ 0.82 &                            64.45 $\pm$ 0.80 \\
 \midrule \multirow{4}{*}{Standard co-training} &   Standard &  \textbf{52.50 $\pm$ 0.82} &           65.32 $\pm$ 0.78 &           \multirow{2}{*}{65.15 $\pm$ 0.80} \\
                                     &  +Standard &  \textbf{51.81 $\pm$ 0.84} &           65.51 $\pm$ 0.77 &                                             \\
                         \cline{2-5} &      Sobel &  \textbf{51.93 $\pm$ 0.82} &           75.18 $\pm$ 0.71 &  \multirow{2}{*}{\textbf{77.86 $\pm$ 0.70}} \\
                                     &    +BagNet &           44.48 $\pm$ 0.81 &  \textbf{78.39 $\pm$ 0.69} &                                             \\
\midrule
 \multirow{4}{*}{Disjoint co-training} &   Standard &  \textbf{52.50 $\pm$ 0.82} &           63.64 $\pm$ 0.80 &           \multirow{2}{*}{64.54 $\pm$ 0.80} \\
                                     &  +Standard &  \textbf{51.81 $\pm$ 0.81} &           64.01 $\pm$ 0.80 &                                             \\
                         \cline{2-5} &      Sobel &  \textbf{51.93 $\pm$ 0.83} &           74.66 $\pm$ 0.74 &  \multirow{2}{*}{\textbf{77.73 $\pm$ 0.67}} \\
                                     &    +BagNet &           44.48 $\pm$ 0.81 &  \textbf{78.14 $\pm$ 0.69} &                                             \\
\bottomrule
\end{tabular}


==> figures/basic_table_cifarsmallsub_pureT.tex <==
\begin{tabular}{llccc}
\toprule
                                  Method &  Prior(s) &               Labeled only &                 \begin{tabular}{c}+Unlabeled \\Self/Co-Training\end{tabular}&                          \begin{tabular}{c} + Standard model \\with Pseudo-labels \end{tabular} \\
\midrule
      \multirow{4}{*}{Self-training} &   Standard &  \textbf{52.50 $\pm$ 0.85} &           64.61 $\pm$ 0.78 &                            64.01 $\pm$ 0.81 \\
                                     &      Canny &           45.66 $\pm$ 0.83 &           52.76 $\pm$ 0.81 &                            55.93 $\pm$ 0.83 \\
                                     &      Sobel &  \textbf{51.93 $\pm$ 0.82} &           63.63 $\pm$ 0.79 &                            64.87 $\pm$ 0.80 \\
                                     &     BagNet &           44.48 $\pm$ 0.82 &           63.77 $\pm$ 0.80 &                            64.45 $\pm$ 0.82 \\
 \midrule \multirow{6}{*}{Co-training} &   Standard &  \textbf{52.50 $\pm$ 0.82} &           63.64 $\pm$ 0.80 &           \multirow{2}{*}{64.54 $\pm$ 0.80} \\
                                     &  +Standard &  \textbf{51.81 $\pm$ 0.81} &           64.01 $\pm$ 0.80 &                                             \\
                         \cline{2-5} &      Canny &           45.66 $\pm$ 0.81 &           62.19 $\pm$ 0.83 &           \multirow{2}{*}{72.60 $\pm$ 0.73} \\
                                     &    +BagNet &           44.48 $\pm$ 0.82 &           72.58 $\pm$ 0.74 &                                             \\
                         \cline{2-5} &      Sobel &  \textbf{51.93 $\pm$ 0.83} &           74.66 $\pm$ 0.74 &  \multirow{2}{*}{\textbf{77.73 $\pm$ 0.67}} \\
                                     &    +BagNet &           44.48 $\pm$ 0.81 &  \textbf{78.14 $\pm$ 0.69} &                                             \\
\bottomrule
\end{tabular}


==> figures/fancy_pretrained_ensemble.tex <==
\begin{footnotesize}
  \def\arraystretch{1.1}
    \addtolength{\tabcolsep}{-1pt}    
    \begin{tabular}{l|ccc|ccc}
      \toprule
      & \multicolumn{3}{c|}{CIFAR-10} & \multicolumn{3}{c}{STL-10} \\
      \midrule 
           Feature Priors &   Model 1 &  Model 2 & \begin{tabular}{c} Stacked \\ Ensemble \end{tabular} & Model 1 &  Model 2 &  \begin{tabular}{c} Stacked \\ Ensemble \end{tabular}\\
      \midrule
      Standard + Standard & 52.54 $\pm$ 0.85 & 51.82 $\pm$ 0.85 & 54.13 $\pm$ 0.88 & 53.73 $\pm$ 0.86 & 55.38 $\pm$ 1.00 & 56.01 $\pm$ 0.94\\
            Sobel + Sobel & 51.94 $\pm$ 0.88 & 53.69 $\pm$ 0.86 & 54.46 $\pm$ 0.92 & 55.49 $\pm$ 0.94 & 55.64 $\pm$ 0.98 & 56.59 $\pm$ 0.96\\
            Canny + Canny & 45.48 $\pm$ 0.84 & 44.19 $\pm$ 0.88 & 46.42 $\pm$ 0.81 & 56.29 $\pm$ 0.92 & 54.99 $\pm$ 0.96 & 57.70 $\pm$ 0.90\\
          BagNet + BagNet & 42.22 $\pm$ 0.80 & 42.56 $\pm$ 0.83 & 44.28 $\pm$ 0.83 & 52.04 $\pm$ 0.92 & 50.34 $\pm$ 0.90 & 52.35 $\pm$ 0.97\\
          \hline
         Standard + Sobel & 52.54 $\pm$ 0.79 & 51.94 $\pm$ 0.82 & \textbf{57.42 $\pm$ 0.84} & 53.73 $\pm$ 0.94 & 55.49 $\pm$ 0.95 & 57.69 $\pm$ 0.95 \\
         Standard + Canny & 52.54 $\pm$ 0.87 & 45.48 $\pm$ 0.81 & 55.70 $\pm$ 0.85 & 53.73 $\pm$ 1.00 & 56.29 $\pm$ 0.94 & 59.24 $\pm$ 0.88 \\
        Standard + BagNet & 52.54 $\pm$ 0.85 & 42.22 $\pm$ 0.80 & 53.65 $\pm$ 0.85 & 53.73 $\pm$ 0.95 & 52.04 $\pm$ 0.90 & 56.03 $\pm$ 0.98 \\
            Sobel + Canny & 51.94 $\pm$ 0.82 & 45.48 $\pm$ 0.85 & 53.30 $\pm$ 0.83 & 55.49 $\pm$ 0.91 & 56.29 $\pm$ 0.94 & 59.54 $\pm$ 0.92 \\
           Sobel + BagNet & 51.94 $\pm$ 0.86 & 42.22 $\pm$ 0.82 & 55.75 $\pm$ 0.83 & 55.49 $\pm$ 0.94 & 52.04 $\pm$ 0.95 & 58.48 $\pm$ 0.96 \\
           Canny + BagNet & 45.48 $\pm$ 0.78 & 42.22 $\pm$ 0.79 & 51.89 $\pm$ 0.87 & 56.29 $\pm$ 0.96 & 52.04 $\pm$ 0.95 & \textbf{59.98 $\pm$ 0.91} \\
      \bottomrule
      \end{tabular}
      
      \addtolength{\tabcolsep}{1pt}    
  \end{footnotesize}


==> figures/pretrained_prior_cifarsmallsub.tex <==
% {('sobel', 'canny'): [0.32935935643458597], ('sobel', 'bagnet'): [0.1838123320257203], ('sobel', 'none'): [0.2640169205826297], ('canny', 'bagnet'): [0.14085278096580656], ('canny', 'none'): [0.226836543650633], ('bagnet', 'none'): [0.38879682081452716]}

% \begin{tabularx}{\linewidth}{l*{5}{X}}
%     \toprule
%             & Standard & Canny & Sobel & BagNet \\ \midrule
%     Standard & --      & 0.227 & 0.264 & 0.389  \\
%     Canny   &         & --    & 0.329 & 0.141  \\
%     Sobel   &         &       & --    & 0.184 \\
%     BagNet  &         &       &       & -- 
% \end{tabularx}

\begin{tabular}{l|cccc}
    \toprule
            & Standard & Canny & Sobel & BagNet \\ \midrule
    Standard & --      & 0.227 & 0.264 & 0.389  \\
    Canny   &         & --    & 0.329 & 0.141  \\
    Sobel   &         &       & --    & 0.184 \\
    BagNet  &         &       &       & --  \\
    \bottomrule
\end{tabular}

==> figures/pretrained_prior_stl10.tex <==
% {('sobel', 'canny'): [0.3931136946867776], ('sobel', 'bagnet'): [0.25929015486380214], ('sobel', 'none'): [0.38138260379750255], ('canny', 'bagnet'): [0.22082345357445393], ('canny', 'none'): [0.308213656969051], ('bagnet', 'none'): [0.3565001294512251]}
\begin{tabular}{l|cccc}
    \toprule
            & Standard & Canny & Sobel & BagNet \\ \midrule
    Standard & --      & 0.308 & 0.381 & 0.357\\
    Canny   &         & --    & 0.393 & 0.220\\
    Sobel   &         &       & --    & 0.259\\
    BagNet  &         &       &       & -- \\
    \bottomrule
\end{tabular}

==> figures/prior_correlations_pure.tex <==
% STL-10: {('canny_self_train', 'canny'): 0.5207705357888011, ('bagnet_self_train', 'bagnet'): 0.5157107784766677, ('sobel_self_train', 'sobel'): 0.6188213879337021, ('control_self_train', 'none'): 0.7276758177406267, ('sobel_bagnet', 'sobel'): 0.5775693718516608, ('sobel_bagnet', 'bagnet'): 0.554039308112243, ('sobel_bagnet_pure', 'sobel'): 0.561900651765842, ('sobel_bagnet_pure', 'bagnet'): 0.5454948237450401, ('canny_bagnet', 'canny'): 0.4920875173062508, ('canny_bagnet', 'bagnet'): 0.5376653917719081, ('canny_bagnet_pure', 'canny'): 0.5176482794195105, ('canny_bagnet_pure', 'bagnet'): 0.5239910387823079}

% {('canny_self_train', 'canny'): 0.6224569949513763, ('bagnet_self_train', 'bagnet'): 0.7591810677405262, ('sobel_self_train', 'sobel'): 0.7594541459270272, ('control_self_train', 'none'): 0.8130664008270849, ('sobel_bagnet', 'sobel'): 0.7062364629121751, ('sobel_bagnet', 'bagnet'): 0.6919896395591723, ('sobel_bagnet_pure', 'sobel'): 0.6856704279164214, ('sobel_bagnet_pure', 'bagnet'): 0.6982682767981885, ('canny_bagnet', 'canny'): 0.5541311693153439, ('canny_bagnet', 'bagnet'): 0.665904273673495, ('canny_bagnet_pure', 'canny'): 0.5554878660722453, ('canny_bagnet_pure', 'bagnet'): 0.6720557767150432}
\begin{tabular}{cc|rr|rr}
    \toprule
    Method                                & Prior   & \begin{tabular}{r} STL-10 Era 0 \\ $r_{Prior, Final}$\end{tabular} & \begin{tabular}{r} STL-10 Era 20 \\ $r_{Prior, Final}$\end{tabular} & \begin{tabular}{r} CIFAR-10 Era 0 \\ $r_{Prior, Final}$\end{tabular} & \begin{tabular}{r} CIFAR-10 Era 20 \\ $r_{Prior, Final}$\end{tabular} \\ \midrule
    \multirow{4}{*}{Self-training}        & Canny   &        0.308               &  0.521 & 0.227 & 0.622\\
                                            & Sobel   &        0.381               &  0.619 & 0.264& 0.759\\
                                            & BagNet  &        0.356               &  0.516 & 0.389 & 0.759\\ \hline
    \multirow{4}{*}{\begin{tabular}{l} Co-training\\Standard\end{tabular}} & Canny   &        0.308               &  0.492 & 0.227 & 0.554\\
                                            & +BagNet &        0.356               &  0.538 & 0.389 & 0.666\\
    \cline{2-6}
                                            & Sobel   &        0.381               &  0.578 & 0.264 & 0.706\\
                                            & +BagNet &        0.356               &  0.554 & 0.389 & 0.692\\\hline
    \multirow{4}{*}{\begin{tabular}{l} Co-training\\Pure\end{tabular}}     & Canny   &        0.308               &  0.518 & 0.227 & 0.556\\
                                            & +BagNet &        0.356               &  0.523 & 0.389 & 0.672\\
    \cline{2-6}
                                            & Sobel   &        0.381               &  0.562 & 0.264 & 0.686\\
                                            & +BagNet &        0.356               &  0.546 & 0.389 & 0.698\\
\end{tabular}

==> icml2022_header.tex <==
\usepackage{graphicx}
\usepackage{psfrag}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{verbatim}
\usepackage{optidef}
\usepackage{mathrsfs}
\usepackage{hyperref}
\usepackage{color}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}

\usepackage{subcaption}
\usepackage{booktabs}
\usepackage{tabularx}
\usepackage{multirow}
\usepackage{float}

% \usepackage[ruled,vlined]{algorithm2e}
% \SetKwInOut{Input}{Input}
% \SetKwInOut{Parameters}{Parameters}

\usepackage[textsize=scriptsize]{todonotes}

\newcommand{\figureinsert}[1]{
    \textcolor{red}{(#1)}
}

\newcommand{\saachi}[1]{\textcolor{blue}{(@saachi: #1)}}
\newcommand{\saachij}[1]{\todo[color=blue!40]{SJ: #1}}

\newcommand{\dimitris}[1]{\todo[color=red!40]{DT: #1}}

\newif\ificml


==> sections/evaluation.tex <==
In this section, we explore combining models with diverse feature priors 
in the presence of unlabeled data using both ensemble and co-training techniques. 

We begin by considering a setting where the unlabeled (and evaluation) data follows 
the same distribution as the labeled data. Thus, while the labeled dataset may 
be small, the models do not encounter significant distribution shift. 

\paragraph{Setup:} For both the CIFAR-10 and STL-10 datasets,
we treat a small fraction of the training set as \emph{labeled}
examples (100 examples per class), another fraction as our validation set
for tuning hyperparameters (10\% of the total training examples), and the 
rest of the training set as our \emph{unlabeled} data. We report our results
on the standard test set of each dataset. Starting from models 
pre-trained on the labeled data using different priors, we evaluate self-training,
ensembling, and co-training techniques. (See Appendix~\ref{app:setup} for 
a full description of our setup and training process.)


\begin{table}
    \begin{subfigure}[b]{\linewidth}
        \begin{center}
            \input{figures/selftrained_ensembles_stlsub10.tex}
        \end{center}
        \caption{STL-10}
        % \vspace{0.5em}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
        \begin{center}
            \input{figures/selftrained_ensembles_cifarsmallsub.tex}
        \end{center}
        \caption{CIFAR-10}
        % \vspace{0.5em}
    \end{subfigure}
    \caption{Ensemble performance when combining \textit{self-trained} models with Standard, Canny, Sobel, and BagNet priors. 
    When two models of the same prior are ensembled, the models are trained with different 
    random initializations.}
    \label{tab:self_trained_ensembles}
\end{table}

\subsection{Diverse priors are still important for ensembling self-trained models}
After self-training our models with different priors on the unlabeled data,
we first revisit the behavior of combining these models using an ensemble (Table TODO). Similar to
Section~\ref{self_trained_ensembles}, we find that prediction diversity
is linked to improved ensemble 
performance. \saachij{Elaborate further after adding the table}

\subsection{Jointly training models with diverse priors through co-training}
\label{sec:ssl}
We then move beyond simply ensembling self-trained models by jointly training the models
on the unlabeled data through co-training. 
We find that using co-training with shape- and texture-based priors can have a large impact on
the test accuracy of the final model (see Table~\ref{tab:basictable} for the full
results and Figure~\ref{fig:summary} for a summary).
Specifically, we observe an improvement of 6.8 percentage points for STL-10 and
13.8 percentage points for CIFAR-10 (Column 5, Table~\ref{tab:basictable}).
This is despite the fact that, when using self-training alone, the standard
model outperforms all other models (Column 4, Table~\ref{tab:basictable}).
This suggests that during co-training, the shape- and texture-biased models
significantly improve each other. 


Moreover, co-training models with diverse priors improves upon simply ensembling them. 
This underlines the importance of 
having the models improve off of each other's pseudo-labels over the course of
co-training. That said, just as in ensembling methods, co-training two standard
 models obtained from different random initializations does not lead to a 
 significant performance improvement, indicating that the diversity of the model
 priors is especially important.
 
 Interestingly, we find that, even when considering a single self-trained model,
 the performance of a standard model can be boosted by choosing a 
 different model with a non-standard prior to generate the pseudo-labels.
 Specifically, we compare the performance of the standard model trained from scratch 
 using pseudo-labels from various self-trained models (Column 5, Table \ref{tab:basictable}). 
 In this setting, using a self-trained shape- or texture-biased model for pseudo-labeling 
 outperforms using a self-trained standard model. This is despite the fact that,
 in isolation, the self-trained standard model has higher accuracy than the self-trained 
 shape- or texure-biased ones (Column 4, Table \ref{tab:basictable}). \saachij{Do we want to keep this section here}
 
We considered an alternative co-training approach where each model is only trained on the
pseudo-labels of the other model rather than on a common pseudo-labeled pool of examples.
We find that this approach leads to a similar, albeit slightly lower final
test accuracy (see Appendix Table~\ref{tab:basictabledisjoint}), demonstrating that 
the overall approach of co-training with
diverse priors is relatively robust to the exact choice of co-training strategy.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/basic_bars.pdf}
    \caption{Final test accuracy of pre-trained, self-trained, and co-trained
        models selecting the best feature prior for each.
        Specifically, the accuracies are based on
        Table~\ref{tab:basictable}: we compare the best of the
        pre-trained models (maximum over Column 3), the best self-training method
        (maximum over the first 4 rows of Column 4), and the best co-training
        method (maximum over the last 3 rows of Column 5).\saachi{Add ensemble to summary bar plot}
    }
    \label{fig:summary}
\end{figure}

\begin{table*}[!ht]
            % \def\arraystretch{1.2}
%\phantom{}
    \begin{subfigure}[b]{\linewidth}
        \begin{center}
            \input{figures/basic_table_cifarsmallsub_pureF.tex}
        \end{center}
        \caption{CIFAR-10}
        \vspace{0.5em}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
        \begin{center}
            \input{figures/basic_table_STLSub10_pureF.tex}
        \end{center}
        \caption{STL-10}
    \end{subfigure}
    \caption{Test accuracy of self-training and co-training methods on STL-10
        and CIFAR-10.
        For each model, we report the original accuracy when trained only
        labeled data (Column 3) as well as the accuracy after being trained on
        pseudo-labeled data (Column 4). (Recall that, for the case of
        co-training pseudo-labeling is performed by combining the predictions of
        both models.) Finally, we report the performance of a standard model
        trained from scratch on the resulting pseudo-labels (Column 5).
        We provide 95\% confidence intervals computed via bootstrap with 5000
        iterations.
}
    \label{tab:basictable}
\end{table*}


\paragraph{Model similarity over co-training.}
To further explore the dynamics of co-training, we evaluate how the correlation
between the predictions of the two models evolves as the eras progress in Figure~\ref{fig:prior_independence_over_time} 
(similarly to the correlation of pre-trained models in Table~\ref{tab:independence}).
We find that the shape- and texture-biased models exhibit low correlation at the
start of co-training, but this correlation increases as co-training
progresses.
This is in contrast to the case of self-training each model on its own, where
the correlation remains relatively low.
It is also worth noting that the correlation appears to plateau at a lower value
when co-training models with distinct feature priors as opposed to co-training
two standard models.
Finally, we find that a standard model trained on the pseudo-labels of other
models correlates well with the models
themselves (see Appendix Table~\ref{tab:independence_after_cotraining}).
Overall, these findings indicate that models trained on each other's
pseudo-labels end up behaving more similarly.

\begin{figure*}[htp]
    \hfill
    \begin{subfigure}[b]{0.44\linewidth}
        \includegraphics[width=\linewidth]{figures/cifarsmallsub_prior_correlations.pdf}
    \caption{CIFAR-10}
    \end{subfigure}
    \hfill 
    \begin{subfigure}[b]{0.44\linewidth}
        \includegraphics[width=\linewidth]{figures/STLSub10_prior_correlations.pdf}
    \caption{STL-10}
    \end{subfigure}
    \hfill 
    \phantom{}
    \caption{Correlation between the correct predictions of shape- and texture-biased models
        over the course of co-training for STL-10 and CIFAR-10. For comparison,
        we also plot the correlation between the predictions when the models
        induced by these priors are individually self-trained, as well as the
        correlation of two standard models when co-trained together.}
    \label{fig:prior_independence_over_time}
\end{figure*}


\section{Using Co-Training to Avoid Spurious Correlations}
\label{sec:spurious}

A major challenge when training models for real-world deployment is avoiding
spurious correlations: associations which are predictive on the training data
but not valid for the actual task.
Examples include predicting the class of an 
object based on its location~\citep{beery2018recognition,xiao2020noise},
or relying on artifacts of the data collection
process~\cite{gururangan2018annotation}.
Since models are typically trained to minimize loss on the training set, they are
quite likely to rely on such spurious correlations~\cite{geirhos2020shortcut}.

In this section, our goal is to leverage diverse feature priors to control the
sensitivity of the training process to such spurious correlations.
Specifically, we will assume that the spurious correlation does not hold on the
unlabeled data (which is likely since unlabeled data is often collected through
a more diverse process).
In this case, if the problematic correlation is not easily captured by one of
the priors, we expect the corresponding model to generate pseudo-labels that are
inconsistent with this association during co-training.
Those pseudo-labels will then steer the more vulnerable model away from 
this correlation. 

\paragraph{Setup.}
We study spurious correlations in two settings.
First, we create a synthetic dataset by tinting each image of the STL-10 labeled
dataset in a class-specific way.
This encourages models to predict using the tint, as it is highly
predictive on the training set.
At the same time, such a prediction rule does not generalize to the test set
where this correlation is absent.

Second, we consider a real-world gender classification task based on
CelebA~\citep{liu2015faceattributes} where hair color (``blond'' vs.\ ``non-blond'') is
predictive on the labeled data but not on the unlabeled and test data.
Specifically, gender and hair color are independent
attributes on the unlabeled dataset, while the labeled dataset consists only of blond females and non-blond
males. Similarly to the synthetic case, the labeled data encourages a prediction rule based only on
hair color.
We use the standard CelebA test set, which consists of roughly $12\%$ blond
females, 
$49\%$ non-blond females, $1\%$ blond males, and $38\%$ non-blond males.
Thus, predicting based on the association ``blond'' $\to$ ``female'' results in
a test accuracy of around 50\%.
See Appendix~\ref{app:datasets} for further details.

\begin{table*}[!ht]
    % \def\arraystretch{1.2}
%\phantom{}
\begin{subfigure}{\linewidth}
\begin{center}
    \input{figures/spurious_table_STLSub10_pureF.tex}
\end{center}
\caption{Tinted STL-10}
\vspace{0.5em}
\end{subfigure}
\begin{subfigure}{\linewidth}
    \begin{center}
        \input{figures/spurious_table_celeba_pureF.tex}
    \end{center}
    \caption{CelebA}
\end{subfigure}
\caption{Test accuracy of self-training and co-training on tinted STL-10 and CelebA,
    two datasets with spurious features (table structure is identical
    Table~\ref{tab:basictable}).
In tinted STL-10, a class-specific tint is added to 
the labeled dataset. In CelebA, the labeled data contains a spurious correlation
between hair color and gender. In both datasets, the spurious correlation is
more easily captured by the BagNet and Standard models over the shape-based ones.
Nevertheless, when co-trained with a shaped-biased model, BagNets are able to
significantly improve their performance, indicating that they rely less on this
spurious correlation. We compute 95\% confidence intervals via 5000 bootstrap
samples.}
\label{tab:spurioussynthetic}
\end{table*}

\paragraph{Performance on datasets with spurious features.}
We evaluate our co-training method along with self-training approaches on the
tinted STL-10 dataset and the CelebA dataset in Table~\ref{tab:spurioussynthetic}.
We find that, when trained only on the labeled data (where the correlation is
fully predictive), both the standard and BagNet models generalize poorly in
comparison to the shape-biased models (see Table~\ref{tab:spurioussynthetic}).
This behavior is expected: the spurious attribute in both datasets is
color-related and hence mostly suppressed by the edge detection algorithms used
to train shape-based models.
Moreover, even after self-training on the unlabeled data (where the correlation
is absent), the performance of the standard and BagNet models does not improve
significantly.

In contrast, when we co-train a BagNet model with a shape-based one, the
BagNet model improves substantially. With Canny/BagNet 
co-training, the resulting BagNet model outperforms its self-training
performance by 42 percentage points on the 
tinted STL-10 dataset and 27 percentage points on the CelebA dataset. 
This improvement can be attributed to the fact that the predictions
of the shape-biased model are not consistent with the spurious correlation on the unlabeled data.  
Hence, by being trained on pseudo-labels from that model, the
BagNet model is forced to rely on alternative, non-spurious features for its predictions.

Interestingly, particularly on the CelebA dataset, the shape-biased model also improves through co-training. 
Specifically, both shape-biased models improve by 4-5 percentage points
over their self-training performance when co-trained with a texture-biased
model.
This indicates that even though the texture-biased model relies heavily on the
spurious correlation, it also captures non-spurious associations that, through
pseudo-labeling, improve the performance of the shape-based model.
These gains are reflected in the performance of the final standard model trained on the combined pseudo-labels. 
In Appendix Table ~\ref{tab:splitceleba}, we find that the gains from
co-training are almost entirely concentrated on input samples
where the spurious correlation does not hold.
This indicates that our method successfully steers the BagNet model away 
from that correlation.

